An Overview of Compressible and Learnable Image Transformation with Secret Key and Its Applications

This article presents an overview of image transformation with a secret key and its applications. Image transformation with a secret key enables us not only to protect visual information on plain images but also to embed unique features controlled with a key into images. In addition, numerous encryption methods can generate encrypted images that are compressible and learnable for machine learning. Various applications of such transformation have been developed by using these properties. In this paper, we focus on a class of image transformation referred to as learnable image encryption, which is applicable to privacy-preserving machine learning and adversarially robust defense. Detailed descriptions of both transformation algorithms and performances are provided. Moreover, we discuss robustness against various attacks.

==> figs/intro_old.tex <==
%The use of images and video sequences has greatly increased because of the rapid growth of the Internet and widespread use of multimedia systems. While many studies on secure, efficient, and flexible communications have been reported~\cite{huang2014apsipatrans, lagendijk2013ieeespmagazine,zhou2014ieeetifs,moo2013nsdi}, full encryption with provable security (like RSA and AES) is the most secure option for securing multimedia data. However, there is a trade-off between security and other requirements such as low processing demand, bitstream compliance, and signal processing in the encrypted domain. Several perceptual encryption schemes have been developed to achieve these trade-offs~\cite{wenjun2003ieeetmlti,ito2008icip,ito2008eusipco,ito2009eurasip,zhenjun2015mtapp,chengqing2017ieeemm,zhang2017opticscomm}. 

%Image encryption prior to image compression is required in certain practical scenarios such as secure image transmission through an untrusted channel provider. Encryption-then-Compression (EtC) systems~\cite{zhou2014ieeetifs,erkin2007eurasip,Nimbokar2014ijca,liu2018ieeebio,osamu2015icassp,kenta2015pcs,Kenta2015ieice,kenta2016bmsb,Kenta2017ieice,warit2018icme,chuman2019ieeetifs} are used in such scenarios. In this paper, we focus on EtC systems with JPEG compression although the traditional way of securely transmitting images is to use a Compression-then-Encryption (CtE) system. Since most studies on EtC systems assumed the use of a proprietary compression scheme incompatible with international compression standards such as JPEG~\cite{zhou2014ieeetifs,liu2018ieeebio,osamu2015icassp,liu2010ieeetip,hu2014icassp,johnson2004ieeetsp}, block scrambling-based image encryption schemes, which are compatible with international standards, have been proposed for EtC systems~\cite{kenta2015pcs,Kenta2015ieice,kenta2016bmsb,Kenta2017ieice,warit2018icme,chuman2019ieeetifs}. 

%A lot of image encryption methods~\cite{zhou2014ieeetifs,zhang2017opticscomm,erkin2007eurasip,Nimbokar2014ijca,liu2018ieeebio,osamu2015icassp,kenta2015pcs,Kenta2015ieice,kenta2016bmsb,Kenta2017ieice,warit2018icme,chuman2019ieeetifs,liu2010ieeetip,hu2014icassp,johnson2004ieeetsp,gaata2016ijmter,yue2012jei} have been proposed for securing image data. However, some of them do not consider the compression to the encryption schemes. A hybrid compression–encryption algorithm~\cite{zhang2017opticscomm} has been proposed to jointly consider both compression and encryption. In this algorithm, an image is compressed and encrypted at the same time. Moreover, various compression-friendly algorithms~\cite{zhou2014ieeetifs,zhang2017opticscomm,erkin2007eurasip,Nimbokar2014ijca,gaata2016ijmter,yue2012jei} have been studied although they do not consider applying them to applications with JPEG compression, such as Social Network Services (SNS) and Cloud Photo Storage Services (CPSS). In~\cite{zhou2014ieeetifs,liu2018ieeebio,osamu2015icassp}, the compression methods for EtC systems have been proposed, but they are not applicable to EtC systems with JPEG compression. Therefore, the works~\cite{kenta2015pcs,Kenta2015ieice,kenta2016bmsb,Kenta2017ieice,warit2018icme,chuman2019ieeetifs} only focus on EtC systems with JPEG compression. 

%In this paper, we present a novel grayscale-based image encryption scheme for EtC systems that enhances security compared with the conventional color-based scheme~\cite{kenta2015pcs,Kenta2015ieice,kenta2016bmsb,Kenta2017ieice}. A grayscale image is an image with a range of shades of gray without color information, where the darkest possible shade is black, and the lightest possible shade is white. In contrast, a grayscale-based image is artificially generated from three color channels of a color image, and pixels in the image have color information. Therefore, the original color image can be reconstructed from the grayscale-based image. Although the conventional grayscale-based image encryption scheme~\cite{warit2018icme,chuman2019ieeetifs}, which is an extension of the color-based EtC systems~\cite{osamu2015icassp,kenta2015pcs,Kenta2015ieice,kenta2016bmsb,Kenta2017ieice}, has been proposed to enhance the robustness against several attacks, such as brute-force and jigsaw puzzle solver attacks~\cite{chuman2017icassp,chuman2017icme,chuman2018ieice}, and also avoid the effect of color subsampling, the compression performance is degraded compared with the color-based image encryption scheme~\cite{osamu2015icassp,kenta2015pcs,Kenta2015ieice,kenta2016bmsb,Kenta2017ieice}. This is because a grayscale-based image is generated from RGB components of a full-color image, so the correlation 

%Consequently,we aim to propose a novel grayscale-based encryption scheme that has almost the same compression performance as non-encrypted images as well as the color-based scheme. We also consider a JPEG quantization table which is especially designed for grayscale-based images. We evaluated the performance of the proposed scheme in terms of the compression performance and security. The results showed that the proposed scheme has almost the same compression performance as the color-based scheme while having almost the same robustness against ciphertext-only attacks as the conventional grayscale-based encryption. 

%The rest of paper is organized as follows. Section II provides a review of the color-based and conventional grayscale-based image encryption schemes used in EtC systems. Section III presents the proposed grayscale-based image encryption and the new quantization table for grayscale-based images. Extensive experimental results including the compression performance and robustness against jigsaw puzzle solver attacks are given in Section IV. Concluding remarks are in Section V.
